Costs and benefits of authentication advice

Authentication security advice is given with the goal of guiding users and organisations towards secure actions and practices. In this paper, we demonstrate that security advice can be ambiguous, contradictory and at times may not even have any clear benefits. We expand on current work by defining a formal approach to identifying costs of security advice and instigate a user study to identify the costs that apply to a large range of authentication advice. We also apply a simple framework for analysing the authentication related security benefits of advice. This allows us to identify costs and benefits for all classes of security advice.

==> Extra info for me/benefits_table_stats.tex <==

% I think the values may be wrong
\begin{tabular}{c|c|c|c|c|c|c|c|}
 RANK&   Attack type         &  Org pos     & Org Neg   & User Pos  &User neg      &total pos & total neg\\\hline 
 R1     &    online         &   19          &   2       &   22      &   2   &       41      &       4  \\
 R2     &    Offline        &   16          &   2       &   16      &   2   &       32      &       4 \\
 R3     &    Eaves          &   11          &   2       &   6       &   2   &       17      &       4  \\
 R4     &    Dupl           &   9           &   1       &   3       &   3   &       12      &       4  \\
 R4     &    endp           &   7           &   0       &   5       &   1   &       12      &       1\\
 R4     &    Phish          &   5           &   0       &   7       &   1   &       12      &       1\\
 R5     &    Side           &   10          &   0       &   1       &   1   &       11      &       1\\  
 R6     &    Soc.eng        &   6           &   0       &   4       &   1   &       10      &       1 \\
 R7     &    unauth         &   9           &   0       &   0       &   0   &       9       &       0\\
 R8     &    Assertion      &   7           &   0       &   0       &   0   &       7       &       0\\
 R9     &    Phys           &   4           &   3       &   0       &   2   &       4       &       5\\
\end{tabular}



%Aside: probabilities from NO policy doc from verizon doc. 
P[side channel attack] = 0.00003836                 R5              

P[theft]= 0.00112                                   R9
    
P[social engineering] = 0.00112                     R6

P[offline guessing] = 0.0014                        R2

P[duplication] = 0.0018                             R4

P[assertion manufacture or modification] = 0.0037   R8

P[unauthorized binding] = 0.0047                    R7

P[online guessing] = 0.0068                         R1

P[phishing] = 0.01889                               R4

P[endpoint compromise] = 0.0196                     R4

P[eavesdropping] = 0.0229                           R3

%P[database of passwords is leaked] = 0.0014 P[user password is guessed in $10^{13}$ guesses] =1
%LOGARITHMIC BUCKETS - 

            green down decrease	        red up increase
Assertion	4	                        0
Phys	    1	                        2
Dupl	    8	                        2
Eaves	    13	                        3
Offline	    28	                        2
Side	    4	                        0
Phish	    7	                        0
Soc.eng	    6	                        0
Online	    34	                        2
endp	    5	                        0
Unauth	    4	                        0

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%How to graph horizontally
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


library(ggplot2)
library(plotrix)
library(reshape2)


df2 <- read.table(text=
"number     attacks            type   
4           Assertion_manufacture       g
1           Physical_theft       g
8           Duplication     g
13          Eavesdropping      g
28          Offline_guessing      g
4           Side_channel_attack    g
7           Phishing     g
6           Social_engineering   g
34          Online_guessing    g
5           Endpoint_compromise   g
4           Unauthorized_binding    g
0           Assertion_manufacture      r
-2           Physical_theft    r
-2           Duplication   r
-3           Eavesdropping     r
-2           Offline_guessing    r
0           Side_channel_attack         r
0           Phishing    r
0           Social_engineering   r
-2           Online_guessing    r
0           Endpoint_compromise      r
0           Unauthorized_binding     r", header=TRUE)

df2$attacks <- stringr::str_replace_all(df2$attacks, '_', ' ')			#replaces underscores with spaces in the variable `attacks' names
df2$attacks <- stringr::str_to_title(df2$attacks)				#makes all the vairables in `attacks' titles so that the first letter is always capitalized. 

#include this line to stop the attack categories swapping order when they are read into a dataframe
df2$attacks <- factor(df2$attacks, levels = unique(df2$attacks)) # create dataframe

p<-ggplot(data=df2, #name of dataframe
	aes(x=attacks,y = number,fill=factor(type))) + 		#x axis is given by `attacks' variable. y axis 	given by `number'. seperated using the variable `type'. 
  	geom_bar(stat="identity", width = 0.6) + 	#If you want the heights of the bars to represent values in the data, use stat="identity". width = width of bars.
  theme(aspect.ratio = 1/1.5)+		#changes length versus width size of plot - I use it to make the width smaller so bars are closer together. 
  coord_flip() # want to graph to be horizontal


q<-p + labs(title="",			#no title
            x="Attack Type", y = "Number of pieces of advice")+		#name axis names
  scale_fill_manual(values=c("#009900", "#FF0000"), #assign colours to different data
labels = c("Decrease chance of attack", "Increase chance of attack"),name = "") + #assign labels for the different data - if automatic ones arent good.  name="" : no title on legend.
  theme(legend.position="top", text = element_text(size=17)) + geom_hline(yintercept=0) #posistion of legend. change size of all text in plot. Include a y intercept at 0 - black line. 

q #to see the graph

ggsave("test.pdf", q, width=8.5, height=7) #save the plot q as test.pdf. specific height and width of the page it is placed on. 

==> Extra info for me/costs_table_stats.tex <==
GRAPH 1
manually read in data to R
#first 6 are org, next 6 are user
cells <- c(7, 0, 40, 2,13, 28, 13, 6,53, 5,12,20)


#Label the columns - x axis
coln <- c("full_per", "full_log", "full_one", "par_per", "par_log", "par_one")

#Label the rows, the comparison bars
rown <- c("Organization", "User")

#Create a matrix of these values
y <- matrix(cells, nrow=2, ncol=6, byrow=TRUE, dimnames=list(rown, coln))

#Plot this matrix. Beside means not a stacked, but side by side. 
barplot(y, ylab="Number of Costs", xlab="Cost Type", col=c("orange", "turquoise" ), beside=TRUE, width=.3, legend=TRUE)


Export: save as pdf


Symbols inserted from latex using copy paste into libreoffice costs_plot4.pdf

libreoffice file.pdf

make font size 22
Replace x axis names with images labels
Make all ctrl a to the top right my 1 cm
Enlarge y axis numbers to font 22
Change orange to boxes
Change legend to organization costs and user costs


GRAPH 2
cells_wo_comp <- c(4, 0, 39, 0,0, 8, 11, 6,53, 5,7,17)

#Label the columns - x axis
coln <- c("full_per", "full_log", "full_one", "par_per", "par_log", "par_one")

#Label the rows, the comparison bars
rown <- c("Organization", "User")

#Create a matrix of these values
y2 <- matrix(cells_wo_comp, nrow=2, ncol=6, byrow=TRUE, dimnames=list(rown, coln))

#Plot this matrix. Beside means not a stacked, but side by side. 
barplot(y2, ylab="Number of Costs", xlab="Cost Type", col=c("orange", "turquoise" ), beside=TRUE, width=.3, legend=TRUE)

%Symbols inserted from latex using copy paste into libreoffice plot_wo_comp4.pdf


STATS ON EACH CATEGORY


==> mindmaps.tex <==
%Brainstorm of Personal Information Advice
\tcbset{colframe=black,colback=white}
\begin{figure*}[t!]
\begin{tcolorbox}
    \centering
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \tikzstyle{block} = [ellipse, minimum width=1cm, minimum height=0.8cm,text centered, draw=black]
\begin{tikzpicture}[grow cyclic, text width=3cm, align=flush center,
    level 1/.style={level distance=2.5cm,sibling angle=73}]

\node[block]{Must not match account information}
     	child { node {Increased computing power for verifier}}
   		child { node {Inconveniences use of a personal system for password generation}}
    	child [xshift=0.5cm, yshift=1.2cm]{ node {$\sim$ Increases risk of forgetting}}
        child { node {$\sim$ Need to pick a new password}}
        child { node {Organizations' time taken to program.}}
    ;
\end{tikzpicture}
        \caption{Personal Information: Must not match account information}
    \end{subfigure}%
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \tikzstyle{block} = [ellipse, minimum width=1cm, minimum height=0.8cm,text centered, draw=black]
\begin{tikzpicture}[grow cyclic, text width=3cm, align=flush center,
    level 1/.style={level distance=2.5cm,sibling angle=60}]
\node[block]{Store history to eliminate reuse}
     	child { node {Increased organization computing power}}
   		child [xshift=0cm, yshift=0.4cm]{ node {Creates an additional security hole}}
    	child { node {Increased risk of forgetting}}
        child { node {Possible multiple attempts until a valid password is chosen}}
        child [xshift=0cm, yshift=-0.5cm]{ node {Organizations' time taken to program}}
        child { node {Need to pick a new password}}
    ;
\end{tikzpicture}
        \caption{Expiry: Store history to eliminate reuse}
    \end{subfigure}%
    \caption{\label{fig:mindmaps}Identifying costs for advice statements. } \label{fig:MatchAcc}
    \end{tcolorbox}
\end{figure*}
